Accelerating String-Key Learned Index Structures via Memoization-based Incremental Training

Learned indexes use machine learning models to learn the mappings between keys and their corresponding positions in key-value indexes. These indexes use the mapping information as training data. Learned indexes require frequent retrainings of their models to incorporate the changes introduced by update queries. To efficiently retrain the models, existing learned index systems often harness a linear algebraic QR factorization technique that performs matrix decomposition. This factorization approach processes all key-position pairs during each retraining, resulting in compute operations that grow linearly with the total number of keys and their lengths. Consequently, the retrainings create a severe performance bottleneck, especially for variable-length string keys, while the retrainings are crucial for maintaining high prediction accuracy and in turn, ensuring low query service latency. To address this performance problem, we develop an algorithm-hardware co-designed string-key learned index system, dubbed SIA. In designing SIA, we leverage a unique algorithmic property of the matrix decomposition-based training method. Exploiting the property, we develop a memoization-based incremental training scheme, which only requires computation over updated keys, while decomposition results of non-updated keys from previous computations can be reused. We further enhance SIA to offload a portion of this training process to an FPGA accelerator to not only relieve CPU resources for serving index queries (i.e., inference), but also accelerate the training itself. Our evaluation shows that compared to ALEX, LIPP, and SIndex, a state-of-the-art learned index systems, SIA-accelerated learned indexes offer 2.6x and 3.4x higher throughput on the two real-world benchmark suites, YCSB and Twitter cache trace, respectively.

==> body/accelerator.tex <==
\section{\liatitle Accelerator}
\label{sec:accelerator}

==> body/cover_letter.tex <==
\onecolumn
\section*{Response to Meta-Reviewer Comments}
%

%
We sincerely appreciate the comments provided by the reviewers and the meta-reviewer, which have significantly contributed to improving our manuscript.
%
Addressing the concerns raised by the meta-reviewer regarding the reproducibility of our work has been a priority.
%
We have taken several steps to ensure that our findings can be readily replicated by others.
%

%
\vspace{1ex}
\noindent
\textbf{Our improvements include:}
%
\begin{enumerate}
%
\item A comprehensive README document outlining the entire procedure for reproducing the experiments
%
\item Scripts designed to replicate the experiments outlined in the paper, facilitating easy execution in real systems
%
\item Detailed instructions on downloading the datasets used in our study, which include Amazon review dataset, MemeTracker dataset, and Twitter cache traces
%
\item Scripts for preprocessing the raw datasets into a format compatible with the used benchmarks and indexes
%
\item Detailed instructions and scripts for synthesizing our SIA accelerator RTL code on the used FPGA.
%
\end{enumerate}
%
Our artifact is available in the following GitHub repository: \bluetext{\url{https://github.com/sia-index/sia}}.
%

%
\vspace{1ex}
\noindent
%
Instructions for reproducing our work, incorporating the aforementioned improvements, are available on the front page of the provided GitHub link or within the \textsf{README.md} file of the repository.
%

%
\vspace{1ex}
\noindent
%
While the core content of the paper remains unchanged, we have made minor revisions such as correcting grammatical errors and including additional citations.
%
Additionally, we have removed colored highlighting from both text and figures.
%


%
%We thank the reviewers for their insightful comments. 
%
%We incorporated all of revision changes requested by the meta reviewer.
%
%To comprehensively respond to the revision requests, we performed extensive experiments and the results are reported in the paper. 
%
% \textbf{In summary (as per meta-reviewer comments), we:}
% \vspace{-1ex}
% \begin{enumerate}
%     \item integrated \sia with two \emph{additional} learned index systems, ALEX~\cite{alex} and LIPP~\cite{lipp}, to demonstrate the generality and wide applicability of the proposed acceleration technique;
%     %
%     \item analyzed the performance implication of index node size and index key type (i.e., integer vs. string); and
%     %
%     \item clarified the unique contributions of this work, distinguishing them from existing and prior techniques.
% \end{enumerate}
% \vspace{-1ex}
%
%In this response letter, we first elaborate on the three major revision points raised by the meta-reviewer, and then provide further details of the revision for the responses to the remainder of the individual reviewer comments. 
%
%In the paper, all the major writing changes are highlighted in \redtext{red}, and all the new or modified figures are boxed in \redbox{red}.
%
%Additionally, we thoroughly proofread the entire manuscript, addressing concerns raised by the reviewers regarding unclear sentences.

% \vspace{1.0ex}

% \vspace{1.5ex}
% \hrule
% \vspace{1.0ex}

% %
% \vspace{1.0ex}
% \noindent
% \textbf{
% \emph{1. Artifact availability.}
% }

% \noindent
% %
% We have improved availability of our artifact in the github repository (https://github.com/sia-index/sia).
% %
% Initially, we provided detailed instructions on downloading the dataset and wrote scripts for preprocessing the dataset into a format compatible with the benchmark and the indexes.
% %
% Subsequently, we wrote scripts to reproduce the experiments outlined in the paper so that users can easily conduct those experiments.
% %
% Moreover, we have supplemented the document to describe all of the above procedures for reproducing the experiments.
% %

% %
% \vspace{1.0ex}
% \noindent
% \textbf{
% \emph{2. Restoration of dataset CDF graph.}}
% \fbox{\textcolor{blue}{
% Section~\ref{sec:evaluation} - Figures~\ref{fig:dataset-cdf}
% }}

% \noindent
% %
% We added back the graph illustrating the key distribution of various dataset used for YCSB and Twitter cache traces.
% %
% Amazon review dataset, MemeTracker dataset, and Twitter cache traces, which we selected as real world datasets exhibit skewed key distributions.
% %
% Learned indexes are designed to learn the cumulative distribution function (CDF) of the dataset, essentially capturing the distribution of the keys.
% %
% Given the skewed distribution of keys, learning becomes more difficult as it moves away from the uniform distribution.
% %
% We showed that \sia performs effectively even with real world datasets with skewed distributions, and to substantiate this claim, we opted to restore the CDF graph of datasets.
% %

% %
% \vspace{1.0ex}
% \noindent
% \textbf{
% \emph{3. Exclusion of experiment on implication of node size.}}
% \fbox{\textcolor{blue}{
% Section~\ref{sec:evaluation}
% }}

% \noindent
% %
% We excluded the evaluation result titled "7.2.9. Implication of Node Size on Throughput".
% %
% As shown in Section~\ref{sec:motivation}, the primary factor contributing to the performance degradation of existing learned indexes is retraining upon modified keys.
% %
% Additionally, Figure~\ref{fig:scalability} shows that this overhead is directly proportional to the number of keys.
% %
% Thus, the implication of node size of a single node on throughput can be deduced without conducting an experiment.
% %
% Due to constraints on space and the relatively low significance of this experiment, We decided to remove the evaluation result from the revised paper.
% %

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% FIRST REVISION %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% %
% \noindent
% \textbf{
% \emph{R3-W3, R4-W1, R4-D1a, R4-D3a: General applicability to other learned indexes.}}
% \fbox{\textcolor{blue}{
% Section~\ref{sec:runtime}; Section~\ref{sec:results} - Figures~\ref{fig:throughput},~\ref{fig:memory-usage-comparison},~\ref{fig:request_dist}}
% }

% \noindent
% %
% We integrated \sia with two additional learned indexes, ALEX~\cite{alex} and LIPP~\cite{lipp}, in addition to SIndex~\cite{sindex}.
% %
% SIndex was the baseline system in the original submission.
% %
% ALEX and LIPP are state-of-the-art learned index systems, leveraging linear regression models as their core learning engines. 
% %
% They also share similar methodologies with SIndex, particularly in terms of node splitting and merging, which are crucial for the management of hierarchical learned index structures.
% %
% To adapt these systems for use with \sia, we replaced their linear regression model training routines with our \sia library calls.
% %
% We elaborated this integration process in Section~\ref{sec:runtime}.
% %
% Additionally, we clarified in Section~\ref{sec:method} that the disparities in how these learned indexes initially build indexes (i.e., top-down vs. bottom-up) do not impact our performance evaluations.
% %
% This is because the initial index building is solely reliant on cold retrainings, a process that does not benefit from the advantages of the proposed incremental index learning algorithm.
% %
% % \highlight{
% % %
% % When building a learned index structure, a hierarchical structure is constructed from key-position batch through bulk loading.
% % %
% % %Bulk load is performed in a top-down manner in ALEX and LIPP, but is performed in a bottom-up manner in SIndex.
% % %, and is usually performed only once when constructing a learned index.
% % %
% % However, there is no memoized matrix when initializing learned index.
% %  %
% % Therefore, acceleration of bulk load is beyond the scope of our focus, and although there are differences between the bulk load mechanisms of ALEX, LIPP, and SIndex, we did not evaluate it.
% % %
% % }
% % %
% Using the three \sia-accelerated systems, we re-performed the same set of experiments for throughput, memory usage, and power efficiency evaluations.
% %
% We observe that the performance results of ALEX-\sia and LIPP-\sia systems follow similar trends to the results in the original submission with SIndex-\sia, which implies the strong applicability of \sia to general string-key based learned index systems.
% %
% The new results are reported at Figure~\ref{fig:throughput}, \ref{fig:memory-usage-comparison}, and \ref{fig:request_dist} in Section~\ref{sec:results}.
% %

% \vspace{1.0ex}
% %
% \noindent
% \textbf{
% \emph{R2-W1: Supported key datatypes - integer learned indexes.}}
% \fbox{\textcolor{blue}{
% Section~\ref{sec:background} - Figure~\ref{fig:li-intstr}
% }}

% \noindent
% %
% \sia can be used for integer-key learned indexes. 
% %
% However, the benefits would be marginal because they experience significantly lower performance bottlenecks due to training because of their arithmetic simplicity. 
% %
% To quantitatively analyze the bottleneck, we compared the throughput of two conventional \emph{non}-learned indexes to that of three learned indexes, and presented the results in Figure~\ref{fig:li-intstr}. 
% %
% Figure~\ref{fig:li-intstr} shows that learned indexes generally offer comparable or higher performance than the two baseline indexes for both integer and string key cases.
% %
% However, the notable observation is that when keys are string, learned indexes perform much worse than the baseline indexes for workloads that contain update queries, which require constant retrainings for index updates. 
% %
% Although these retrainings impose marginal performance overhead when keys are integers, retrainings for string keys are severe performance bottleneck, cancelling the performance benefits of learned indexes.
% %
% For the sake of demonstration and quantification purposes, we still incorporated \sia with integer-key learned index such as ALEX, LIPP, or XIndex~\cite{xindex} and conducted performance evaluation.
% %
% For an insertion ratio of 25\%, we observe a 9.3\% improvement, and for an insertion ratio of 50\%, we observe only 17.3\% improvement in throughput compared to the baseline index.
% %
% These gains appear modest when contrasted with the significant performance improvement when accelerating string-key learned indexes.
% %
% Motivated by this result, we focused on accelerating the string-key learned indexes in this work. 
% %
% \vspace{1.0ex}

% %
% \noindent
% \textbf{
% \emph{R2-W2: Performance implication of node size.}}
% \fbox{\textcolor{blue}{
% Section~\ref{sec:results} - Figure~\ref{fig:threshold-sweep}}}

% \noindent
% %
% The model splitting alters the distribution of keys across nodes without affecting the total key count.
% %
% This means that the overall computational load for training remains the same, incurring minimal impact on overall performance.
% %
% To validate this, we conducted an experiment assessing throughput variations with different node sizes. 
% %
% Figure~\ref{fig:threshold-sweep} reports the results that varies the node size. The results show that \sia-accelerated system obtain similar benefits with small-size leaf nodes. % have minimal effect on both the baseline and \sia-accelerated SIndex systems.
% %
% \vspace{1.0ex}

% %
% \noindent
% \textbf{
% \emph{R2-W4: Novelty. }}
% \fbox{\textcolor{blue}{
% Section~\ref{sec:linear-regression-training}}}

% \noindent
% %
% Apologies for any confusion caused, it is indeed true that QR decomposition (QRD) is a well-established technique commonly used in solving linear equations, and we do not intend to claim novelty from it.
% %
% This paper instead makes two contributions: (1) proposing a modified QRD algorithm, which exploits computation reuse by leveraging its computational partitionability, and the incremental index learning mechanism customized for learned index systems that receive constant update queries over time; and (2) developing a novel learned index training acceleration technique, leveraging the aforementioned algorithmic insight to enable retraining process offloading onto an FPGA accelerator.
% %
% We have made this distinction clear in Section~\ref{sec:linear-regression-training} to prevent any misunderstanding.
% %

% \vspace{1.0ex}

% \vspace{1.5ex}
% \hrule
% \vspace{1.0ex}

% %
% \noindent
% \textbf{
% \emph{R3-W1, R4-W3, R4-D3c: Implication of request distribution on \sia's performance.}}
% \fbox{\textcolor{blue}{
% Section~\ref{sec:results} - Figure~\ref{fig:request_dist}
% }}

% \noindent
% %
% We evaluated the throughput exhibited by ALEX, LIPP, and SIndex, and \sia-accelerated learned indexes using six request distributions, as used in prior works~\cite{bourbon, gadget-eurosys}.
% %
% These request distributions include skewed distributions such as \emph{zipfian},  \emph{hotspot}, and \emph{exponent}, where node splits are more frequent due to the higher frequency of key insertion within a narrow range.
% %
% Nevertheless, we observe that the learned index systems accelerated with \sia consistently outperform learned index baselines across all request distributions including skewed request distributions.
% %
% The results are shown at Figure~\ref{fig:request_dist} in Section~\ref{sec:results}.
% %

% %
% \vspace{1.0ex}



% %
% \noindent
% \textbf{
% \emph{R2-W3: Clarity of Figure~\ref{fig:scalability} and Figure~\ref{fig:incremental-sindex-scalability}.}}
% \fbox{\textcolor{blue}{
% Section~\ref{sec:scalability-analysis} - Figure~\ref{fig:scalability}; Section~\ref{sec:lia-algorithm} - Figure~\ref{fig:incremental-sindex-scalability}
% }}

% \noindent
% %
% Apologies for the confusion. 
% %
% In Figure~\ref{fig:scalability} and Figure~\ref{fig:incremental-sindex-scalability}, the results were collected on a ``running'' learned index system, which progressively receives additional keys added to the index. 
% %
% We conducted such an experiment four times as we change the key length from 16 to 96. 
% %
% To clarify this experimental methodology, we modified Figure~\ref{fig:scalability} and Figure~\ref{fig:incremental-sindex-scalability} with an arrow with the label, ``Time'', and revised the caption accordingly. 
% %
% \vspace{1.0ex}



% %
% \noindent
% \textbf{
% \emph{R3-W2: Concurrent operations.}}
% \fbox{\textcolor{blue}{
% Section~\ref{sec:method}
% }}

% \noindent
% %
% For concurrency support, we leverage existing techniques proposed by prior works, XIndex and SIndex. 
% %
% They ensure consistent index structure across multiple threads with read-copy-update and fine-grained locks.
% %
% % Learned indexes accelerated with \sia also utilize concurrent operations same with those proposed by XIndex and SIndex.
% %
% % Also, given that the public implementations of ALEX and LIPP lack support for concurrency, we adopted the same concurrency mechanisms.
% %
% Furthermore, \sia remains orthogonal to concurrency concerns because, as in the prior works, \sia-accelerated systems invoke the retraining processes ``atomically'' without having any interventions with other retrainings.  
% %
% \vspace{1.0ex}

% %
% \noindent
% \textbf{
% \emph{R4-D1b: Why FPGA. }}
% \fbox{\textcolor{blue}{
% Section~\ref{sec:results} - Figure~\ref{fig:power_consumption}
% }}

% \noindent
% %
% We leverage FPGAs for \sia due to two main reasons: (1) superior power efficiency compared to GPUs (Figure~\ref{fig:power_consumption}), and (2) reconfigurability in comparison to ASICs.
% %
% While the cost of FPGAs may not be lower than that of GPUs, we attribute this disparity to the distinct supply and demand of these two hardware.
% %
% However, in scenarios such as large-scale data centers using FPGAs~\cite{cloud-fpga, brainwave:isca:2018}, economies of scale can reduce costs, realizing advantages in both hardware affordability and power efficiency.
% %
% In contrast to ASICs, FPGAs possess the flexibility to reconfigure for different key lengths, offering a distinct advantage.
% %
% For these reasons, we opt to employ FPGAs as an acceleration platform.
% %
% \vspace{1.0ex}

% %
% \noindent
% \textbf{
% \emph{R4-W2, R4-D2a, R4-D2b: Security and performance implications of lazy deletion. }}
% \fbox{\textcolor{blue}{
% Section~\ref{sec:lazy-deletion}; Section~\ref{sec:results} - Table~\ref{tab:lazy-deletion-impact}
% }}

% \noindent
% %
% We provided further clarification regarding lazy deletion in Section~\ref{sec:lazy-deletion}.
% %
% Despite using lazy deletion, key and value data are removed immediately, while the memoized $R$ matrix containing the information about the deleted key is still used for following incremental retrainings and it is eliminated from system whenever a cold training is triggered.
% %
% Note that the $R$ matrices do not carry any semantic information, and also cannot be used to reproduce the original key matrix since there is no $Q$ matrix stored in the system. 
% %
% Consequently, lazy deletion does not allow attackers to access any key/value data, thus not introducing any new security vulnerabilities.
% %
% Disjointly, the lazy deletion approach may have implications on the hierarchical structure of learned indexes since it could incur more splits and less merges. 
% %
% However, as reported in Table~\ref{tab:lazy-deletion-impact}, the performance overhead of this approach is negligible, which peaks at only 4.6\%.
% %
% \vspace{1.0ex}

% %
% % \noindent
% % \textbf{
% % \emph{R4-D2-b: Structural impact of lazy deletion. }}
% % \fbox{\textcolor{blue}{
% % Section~\ref{???}; Page~\pageref{???}
% % }}

% % \noindent
% % %
% % \todo{}{need contents}
% % %
% % \vspace{1.0ex}

% %
% \noindent
% \textbf{
% \emph{R4-D3b: On-chip memory usage of \sia. }}
% \fbox{\textcolor{blue}{
% Section~\ref{sec:results} - Figure~\ref{fig:memory-usage-comparison}}
% }

% \noindent
% %
% Given the flexibility of the number of keys per node in learned indexes, it is crucial to allocate adequate on-chip memory space.
% %
% Hardware accelerator of \sia should hold the keys to be learned in its on-chip memory and clear them after the calculation is done.
% %
% It can store about 12,000 keys by using 0.5MB out of the available 8.2MB on-chip memory in the FPGA (Table~\ref{tab:fpga}).
% %
% On average, learned indexes utilize 12.6\% of the on-chip memory, peaking at 86.2\%.
% %
% Meanwhile, for off-chip memory, we use DDR memory with sufficient capacity.
% %
% Figure~\ref{fig:memory-usage-comparison} shows off-chip memory usage comparison results between \sia-accelerated learned index and the conventional baselines.
% %
% \vspace{1.0ex}

% %
% \noindent
% \textbf{
% \emph{R4-D3d: In-depth analysis of power consumption. }}
% \fbox{\textcolor{blue}{
% Section~\ref{sec:results} 
% - Figure~\ref{fig:power_consumption}
% }}

% \noindent
% %
% To show the impact of computation phases in learned indexes (e.g., cold training, incremental training, non-training), we expanded the system power consumption measurement, presenting the average, minimum, and maximum power consumption for each element and operation of CPU-only, CPU-GPU, and CPU-FPGA systems.
% %
% CPU tries to maximize resource utilization for the inference regardless of the phases, resulting in minimal power fluctuations.
% %
% Conversely, the GPU exhibits more variability in the results due to its demand-based allocation of computational resources for training.
% %
% We observe that \sia's CPU-FPGA accelerated system requires the least power consumption since the FPGA offers orders-of-magnitude higher power efficiency compared to alternatives.
% %
% Moreover, we also observe that power fluctuations resulting from phase changes are negligible, attributed to the inherently low-power nature of FPGA acceleration. 
% %
% Figure~\ref{fig:power_consumption} reports the detailed results.
% %
% \vspace{1.0ex}


%
% The following line is commented out because it created latex compilation error
% \noindent\sectionlink{Section~\ref{sec:motivation}; Page 2} 

\twocolumn
